Collaborative Agents for Automated Program Repair in Ruby

Automated Program Repair (APR) has advanced rapidly with Large Language Models (LLMs), but most existing methods remain computationally expensive, and focused on a small set of languages. Ruby, despite its widespread use in web development and the persistent challenges faced by its developers, has received little attention in APR research. In this paper, we introduce RAMP, a novel lightweight framework that formulates program repair as a feedback-driven, iterative process for Ruby. RAMP employs a team of collaborative agents that generate targeted tests, reflect on errors, and refine candidate fixes until a correct solution is found. Unlike prior approaches, RAMP is designed to avoid reliance on large multilingual repair databases or costly fine-tuning, instead operating directly on Ruby through lightweight prompting and test-driven feedback. Evaluation on the XCodeEval benchmark shows that RAMP achieves a pass@1 of 67% on Ruby, outper-forming prior approaches. RAMP converges quickly within five iterations, and ablation studies confirm that test generation and self-reflection are key drivers of its performance. Further analysis shows that RAMP is particularly effective at repairing wrong answers, compilation errors, and runtime errors. Our approach provides new insights into multi-agent repair strategies, and establishes a foundation for extending LLM-based debugging tools to under-studied languages.

==> section/introduction-old.tex <==
\section{Introduction}

% \Nikta{Debugging and fixing software bugs remain some of the most time-consuming and error-prone tasks in software development \cite{weber2025understanding, lee2024unified}. While traditional Automated Program Repair (APR) techniques have shown promise \cite{renzullo2025automated, dikici2025advancements}, recent advances in Large Language Models (LLMs) have opened up new possibilities for more flexible, context-aware solutions \cite{yang2025survey, sun2025empirical, li2025context}. However, most existing LLM-based APR approaches face significant limitations \cite{yang2025survey, sun2025empirical, zhang2024systematic, renzullo2025automated, huang2024evolving, zhang2023survey}. They are resource-intensive and difficult to reproduce: fine-tuning requires large GPU budgets, while inference pipelines incur high token costs that make real-world deployment challenging \cite{yang2025survey, zhang2023survey}. Evaluation practices remain narrow, focusing mainly on the number of bugs fixed while overlooking runtime and efficiency, which hinders fair comparison \cite{yang2025survey, zhang2023survey}. Moreover, most studies still rely on traditional benchmarks such as Defects4J, QuixBugs, and BFP, which, although well-established, limit the exploration of newer and more diverse datasets \cite{zhang2024systematic}. Finally, language coverage is highly skewed toward Java, Python, and C, while widely used languages such as Ruby remain largely underexplored ~\cite{zhang2024systematic}.}

% \Nikta{This gap is concerning because Ruby developers continue to face persistent challenges related to debugging, test writing, and ensuring application correctness \cite{akbarpour2025unveiling}. Prior empirical studies of the Ruby ecosystem, drawing on Stack Overflow discussions and developer survey data, reveal recurring pain points \cite{akbarpour2025unveiling}. Notably, 42.13\% of experienced developers report that \textit{Application Quality and Security} is difficult, underscoring ongoing issues such as handling method and parameter errors, implementing validation practices, and writing reliable tests. This category alone accounted for 23.28\% of all developer questions and showed a statistically significant increasing trend over time, highlighting growing concern within the community \cite{akbarpour2025unveiling}. Yet, despite the frequency and severity of these issues, Ruby lacks intelligent, automated support systems for program repair and debugging. Most established APR benchmarks and large-scale evaluations continue to target Java, Python, and C, leaving Ruby notably absent \cite{zhang2023survey}.}

% \FHF{I still dont quite like the first 2 paragraphs of intro. The significance is still not bold. }

Debugging and fixing software bugs remain some of the most time-consuming and error-prone tasks in software development \cite{weber2025understanding, lee2024unified}. While traditional Automated Program Repair (APR) techniques have shown promise \cite{renzullo2025automated, dikici2025advancements}, recent advances in Large Language Models (LLMs) have opened up new possibilities for more flexible, context-aware solutions \cite{yang2025survey, sun2025empirical, li2025context}. However, most existing LLM-based APR approaches face significant limitations \cite{yang2025survey, sun2025empirical, zhang2024systematic, renzullo2025automated, huang2024evolving, zhang2023survey}, being resource-intensive as fine-tuning requires large GPU budgets, while inference pipelines incur high token costs that make real-world deployment challenging \cite{yang2025survey, zhang2023survey}. Evaluation practices remain narrow, overlooking runtime and efficiency, which hinders fair comparison \cite{yang2025survey, zhang2023survey}. Moreover, 
% most studies still rely on traditional benchmarks such as Defects4J, QuixBugs, and BFP, which, although well-established, limit the exploration of newer and more diverse datasets \cite{zhang2024systematic}. Finally, 
language coverage is highly skewed toward Java, Python, and C, while widely used languages such as Ruby remain largely underexplored ~\cite{zhang2024systematic}. \Nikta{This gap is notable given Ruby’s practical significance. Widely used for web applications and with over two million projects on GitHub, Ruby has been used in major platforms such as Airbnb, GitHub, and Shopify \cite{chandran2020correlative, kaleba2022you}. Backed by a community of more than a million developers, its broad adoption underscores the need to extend APR research to this influential yet underexplored language.}
\FHF{Add a few sentences about significance of ruby, where it is used and its number of developers. }

This gap is concerning because Ruby developers continue to face persistent challenges related to debugging, test writing, and ensuring application correctness \cite{akbarpour2025unveiling}. Prior empirical studies of the Ruby ecosystem, drawing on Stack Overflow discussions and developer survey data, reveal recurring pain points for various aspects, such as handling method and parameter errors \cite{akbarpour2025unveiling}. 
% Notably, 42.13\% of experienced developers report that \textit{Application Quality and Security} is difficult, underscoring ongoing issues such as handling method and parameter errors, implementing validation practices, and writing reliable tests. This category alone accounted for 23.28\% of all developer questions and showed a statistically significant increasing trend over time, highlighting growing concern within the community \cite{akbarpour2025unveiling}. 
Yet, 
% despite the frequency and severity of these issues, 
Ruby lacks intelligent, automated support systems for program repair and debugging. Most established APR benchmarks and large-scale evaluations continue to target Java, Python, and C, leaving Ruby notably absent \cite{zhang2023survey}.

Attempts to broaden APR beyond traditional settings still fall short for Ruby. For example, \textsc{LANTERN} \cite{luo2025unlocking} is notable for being evaluated on XCodeEval benchmark \cite{khan2024xcodeeval} and including Ruby, but its reliance on large multilingual repair databases makes it unsuitable for single-language scenarios with limited data. Meanwhile, \textsc{ChatRepair} \cite{xia2024automated} represents an efficient LLM-based repair approach, but it was not evaluated on Ruby and only provides raw execution results to the model, offering minimal feedback and little support for iterative refinement. These examples highlight the broader challenge: no prior system delivers Ruby-focused, multi-agent, feedback-rich repair.

To address these limitations, we introduce \textbf{RAMP}: \textit{\textbf{R}uby \textbf{A}utomated \textbf{M}ulti-agent \textbf{P}rogram repair}, a lightweight, feedback-driven framework that models APR as an iterative repair loop. RAMP decomposes the APR process into specialized roles, including a \texttt{Programmer Agent}, \texttt{Test Designer}, \texttt{Test Executor}, and \texttt{Feedback Integrator}. Starting from a buggy program and problem context, RAMP leverages specialized agents to reflect on the source of errors, generate guiding tests, propose candidate fixes, and validate them through execution feedback. Candidate repairs are iteratively refined until they either pass the generated tests and the benchmark’s hidden suite or the iteration budget is exhausted. 
This multi-agent workflow enables deeper semantic reasoning than single-agent baselines while remaining cost-efficient. Unlike prior systems that rely on large multilingual databases or costly fine-tuning, RAMP operates directly on Ruby code through lightweight prompting and test-driven feedback. By eliminating the need for resource-heavy training pipelines and cross-language translation, it achieves strong repair performance while keeping computation practical for the understudied language, Ruby.

On the XCodeEval benchmark \cite{khan2024xcodeeval}, RAMP attains the best Pass@1 on Ruby (67\%), outperforming LANTERN (61.7\%) and prompting baselines, and converges by iteration~5. Ablation studies show that test generation and self-reflection are pivotal and removing them reduces accuracy by 18.1\% and 19.3\%.
In terms of failure categories defined by XCodeEval, RAMP is especially effective at repairing programs that initially produced WRONG\_ANSWER outputs (i.e., incorrect but executable results, 68.5\% repaired), followed by COMPILATION\_ERROR cases (programs that failed to compile, 66.7\% repaired) and RUNTIME\_ERROR cases (programs that crashed during execution, 60.4\% repaired) but struggles with resource-related failures and advanced categories such as binary search, bitmasks, and matrices. \Nikta{These results highlight RAMP’s effectiveness across diverse bug types and its efficiency in converging quickly, underscoring its promise as a practical solution for automated program repair in Ruby.}
\FHF{Maybe end here with a positive aspect of ramp? its significance.}

In summary, the key contributions of this paper include:
\begin{itemize}
\item \textbf{Introducing RAMP}, the first Ruby-focused APR framework that leverages a lightweight, multi-agent design to enable iterative, feedback-driven program repair without relying on large multilingual databases or fine-tuning.
\item \textbf{Formulating APR as a test-guided repair loop}, where specialized agents collaborate through self-reflection, test generation, candidate repair, and execution feedback, enabling deeper semantic reasoning while remaining cost-efficient.
% \item \textbf{Conducting the first systematic evaluation of APR on Ruby} using the XCodeEval benchmark and identifying the strengths of RAMP. \FHF{Not sure if third item is a contribution.}
{\item \textbf{Releasing all scripts and experimental results} as open source to support replication and future research \footnote{\url{https://osf.io/9kgha/?view_only=72cd13e3bda3439ea8549e319544a001}}.}
\end{itemize}

% We now outline the key research questions that guide our study. These questions are designed to evaluate RAMP’s effectiveness, analyze the contribution of its components, and assess its performance across different dimensions of the repair task.

% \textbf{RQ1: How does RAMP perform in comparison to other APR methods?}
% To evaluate the effectiveness of RAMP, we compare it against representative baselines from prior APR approaches. These include zero-shot prompting, which tests whether an LLM can repair code directly from a task description without guidance; few-shot prompting, which provides exemplar bug–fix pairs as demonstrations; self-planning, which equips the model with structured repair plans before patch generation; self-collaboration, where multiple model instances iteratively critique and refine candidate repairs; and LANTERN \cite{}. RAMP achieves the highest Pass@1 on Ruby at \textbf{67\%}, outperforming LANTERN (61.7\%) and all prompting-based baselines, while also converging faster (by iteration~5) than competing approaches.

% \textbf{RQ2: How do the different agents in RAMP contribute to its overall effectiveness?}  
% Beyond measuring aggregate performance, it is important to understand how each agent within RAMP contributes to the framework’s success. We therefore examine the role of individual agents in driving repair outcomes, isolating their impact on repair success rates and identifying where their contributions are most critical. In particular, we pay close attention to the Test Designer, since the quality and relevance of the generated test cases directly influence the accuracy of fault localization, the effectiveness of feedback, and ultimately the correctness of the final patch. Ablations show that both test generation and self-reflection are critical and removing them reduces Pass@1 by up to 18–19\%, demonstrating their central role in guiding accurate repairs.

% \textbf{RQ3: How do prompting strategies and refinement iterations influence RAMP’s repair performance?}  
% The design of prompts and the use of iterative refinement play a crucial role in determining the quality of program repair. To understand these effects, we investigate how different prompting strategies, such as Chain-of-Thought and Structured Chain-of-Thought, shape the reasoning process of RAMP’s agents and impact repair accuracy. We also analyze the contribution of various prompt components, for example, including sample inputs and outputs, to evaluate whether such auxiliary information strengthens fault localization and patch correctness or instead introduces unnecessary complexity. Finally, we examine the role of iterative refinement, assessing how successive repair attempts improve solution quality and whether diminishing returns emerge after a certain number of iterations. Few-shot Chain-of-Thought yields the best performance (+2.1\% over SCoT), input–output specifications are essential (-10.5\% when omitted), and most solvable tasks are repaired in the first few iterations, with performance plateauing around 66.5\% cumulative Pass@1 by iteration~11.

% \textbf{RQ4: How does RAMP perform across tasks of varying difficulty, subject domains, and initial execution outcomes?}  
% To evaluate the generality and robustness of RAMP, we analyze its performance under diverse task conditions. First, we study how repair success varies with problem difficulty, leveraging the benchmark’s difficulty scores to determine whether RAMP is more effective on simpler bugs or can scale to harder cases. We also assess performance across subject domains by grouping tasks according to benchmark-provided tags, enabling us to examine whether RAMP exhibits domain-specific strengths or weaknesses. Finally, we compare execution outcomes before and after repair: contrasting the behavior of buggy programs against their post-repair versions highlights RAMP’s ability to transform failing or partially correct executions into fully passing ones. RAMP excels on easier problems and common error types, repairing 68.5\% of WRONG\_ANSWER and 66.7\% of COMPILATION\_ERROR cases, but struggles with resource-related failures and advanced categories such as binary search, bitmasks, and matrices.








% Debugging and fixing software bugs remain one of the most time-consuming and error-prone tasks in software development \cite{weber2025understanding, lee2024unified}. While traditional Automated Program Repair (APR) techniques have shown promise \cite{renzullo2025automated, dikici2025advancements}, recent advances in Large Language Models (LLMs) have opened up new possibilities for more flexible, context-aware solutions \cite{yang2025surveyllmbasedautomatedprogram, sun2025empirical, li2025context}. However, most existing LLM-based APR approaches rely on single-turn prompting, procedural pipelines, or fine-tuned models where fine-tuning is costly, static, and difficult to generalize, resulting in limited adaptability and a lack of dynamic reasoning~\cite{sun2025empirical}.

% Despite rapid progress across fine-tuning, prompt engineering, procedural workflows, and agentic frameworks, current approaches to APR still face fundamental limitations.  

% Fine-tuning delivers the highest patch accuracy by embedding domain knowledge into the model \cite{huang2022codet5,jiang2021cubert,vulmaster2024,repaircat2024}, but at the cost of massive GPU consumption, loss of general-purpose coding ability, and dependence on large curated datasets. Parameter-efficient tuning \cite{hu2021lora,repairllama2024,morepair2024} and distillation \cite{knod2023,distilrr2024,narrepair2024} alleviate resource demands, yet their success hinges on careful adapter design and data diversity—constraints that are rarely satisfied in real-world projects. 

% Prompt-based methods, while attractive for their simplicity, are fragile. Zero-shot repair is highly prompt-sensitive \cite{alpharepair2023,fan2023codex,tian2023chatgpt}, and even with examples, the effectiveness depends on manual heuristics and prompt length limits \cite{xia2023fewshot,gao2023retrieval,ahmed2023exemplar,cedar2024}. Supplying too much or poorly chosen context often degrades accuracy, and most retrieval pipelines lack adaptive mechanisms to balance relevance against overhead \cite{rlce2023,trap2023,dsrepair2023,d4c2023,appatch2023,traceprompt2023}.  

% Procedural repair frameworks increase reproducibility by structuring repair into scripted loops of retrieval and feedback \cite{chatrepair2023,thinkrepair2023,rex2023,contrastrepair2023}. However, they are rigid, relying heavily on handcrafted control flows and manually selected feedback. These pipelines scale poorly when applied to large repositories or complex semantic bugs, as each additional artifact expands prompt size and cost \cite{cref2023,hula2023,drcodepilot2024,agentless2023,ragfix2023,kgcompass2023,repilot2023,formhe2023,predicatefix2023,llm4cve2023}.  

% Agentic repair frameworks hold the greatest promise but remain immature. Current systems such as SWE-Agent \cite{wei2023sweagent}, OpenHands \cite{widyasari2024openhands}, AutoCodeRover \cite{zhang2024autocoderover}, RepairAgent \cite{dong2023repairagent}, and LANTERN \cite{luo2025unlocking} demonstrate selective tool use and cross-language translation for boosting repair rates. Yet they often overlook cost control, waste resources on unproductive branches, and suffer from brittle context management. Their autonomy introduces new risks, as agents may loop indefinitely, apply unsafe edits, or degrade latency beyond continuous integration requirements.

% Ruby developers continue to face persistent challenges related to debugging, test writing, and ensuring application correctness \cite{akbarpour2025unveiling}. Prior works identified pain points in the Ruby ecosystem through empirical analysis of Stack Overflow posts and developer survey \cite{akbarpour2025unveiling}. 

% They report that among experienced developers, 42.13\% found \textit{Application Quality and Security} to be difficult, which highlights recurring issues such as handling method and parameter errors, validation practices, and writing tests.
% This issue also accounted for 23.28\% of all developer questions and showed a statistically significant increasing trend over time, suggesting a growing concern in the community \cite{akbarpour2025unveiling}. Despite the frequency and difficulty of these issues, Ruby lacks intelligent, automated support systems for program repair and debugging, particularly compared to languages such as Java or Python \FHF{CITE}.

% Taken together, these shortcomings highlight a critical gap: no existing framework simultaneously balances efficiency, robustness, and scalability while remaining compatible with real-world CI/CD workflows. This motivates our work, which unifies strengths across categories—combining lightweight parameter-efficient adaptation with adaptive context retrieval, structured yet flexible feedback loops, and cost-aware agentic planning—to move toward practical, low-latency, and reliable APR.

% To address these limitations, we introduce \textbf{RAMP}: \textit{Ruby Multi-Agent Program repair}, a novel framework that leverages a team of collaborative, LLM-driven agents to iteratively detect, reason about, and repair buggy Ruby code. RAMP decomposes the APR process into specialized roles, including a \texttt{Programmer}, \texttt{Test Designer}, \texttt{Test Executor}, and \texttt{Feedback Integrator}. Each agent operates based on natural language prompts, structured coordination, and test-driven feedback to collectively repair code candidates. \FHF{Add a few sentences, emphasize on what is new compared to prior work. You do not only apply reflexion or other frameworks on Ruby. what is your novelty?}

% RAMP is tailored for Ruby, a dynamically typed and often under-studied language in the APR literature. By integrating prompting strategies such as Chain-of-Thought, Reflexion, and test-aware reasoning, the framework enables deeper understanding of code behavior and guided iterative repair. Preliminary results demonstrate that the multi-agent design improves repair success rates compared to single-agent baselines, especially in scenarios involving subtle logic errors or incomplete test coverage.
% RAMP introduces a multi-agent, feedback-driven architecture that iteratively improves code via test generation and validation—offering greater flexibility and robustness, especially in dynamic languages like Ruby.







% \FHF{See if you can discuss these issues in the paper based on your findings. A good point would be thinking if any of these issues are also found in the dataset and your results support them. Then you can cite youe previous paper and discuss the results. Ofcourse, if they are relevant!}

% using frameworks like RSpec. Additionally, 


% \FHF{Add a few sentences about prior work. What they have done? what is the gap in the literature that you are addressing in your work? See the outline from Linked IN post that I sent on Slack.}



% \FHF{revise this paragraph after we have finished designing all RQs and experiments. }






